Constructive Separations from Gate Elimination

Gate elimination is the primary technique for proving explicit lower bounds against general Boolean circuits, including Li and Yang's state-of-the-art $3.1n - o(n)$ bound for affine dispersers (STOC 2022). Every circuit lower bound is implicitly existential: every circuit that is too small to compute $f$ must err on some input. This raises a natural question: are these lower bounds \emph{constructive}? That is, can we efficiently produce such errors? Chen, Jin, Santhanam, and Williams showed that constructivity plays a central role in many longstanding open problems in complexity theory, and explicitly raised the question of which circuit lower bound techniques can be made constructive (FOCS 2021). We show that a variety of gate elimination arguments yield refuters -- efficient algorithms that, when given a circuit that is too small to compute a function $f$, produce an input on which the circuit errs. Our results range from elementary lower bounds for $XOR$ and the multiplexer to more sophisticated arguments for affine dispersers. Underlying these results is a shift in perspective: gate elimination arguments \emph{are} algorithms. Each step either simplifies the circuit or reveals a violation of some structural or functional property, from which, with a little additional work, explicit counterexamples can be extracted. We further strengthen the $XOR$ result to handle circuits that \emph{match} the lower bound: given any DeMorgan circuit of size $3(n-1)$ that fails to compute $XOR_n$, we can efficiently produce a counterexample. While refuters follow from the gate elimination arguments themselves, this refinement requires a complete characterization of the set of optimal circuits computing $XOR$ -- a requirement rarely met by other explicit functions.

==> images/tikz/xor-checker-proof/xor-proof-settings.tex <==
\tikzset{node/.style={circle, draw, minimum size=0.75cm}}
\tikzset{mnode/.style={circle, draw, dashed,minimum size=0.75cm}}
\tikzset{output/.style={circle, node contents = {}}}
\tikzset{padding/.style={circle, node contents = {}}}
\tikzset{e/.style={thick}}
\tikzset{w/.style={thick, dashed}}
\tikzset{node distance = 0.75cm}
\tikzset{>=latex}
